On the optimality of Shapley mechanism for funding public excludable goods under Sybil strategies

In the realm of cost-sharing mechanisms, the vulnerability to Sybil strategies -- also known as false-name strategies, where agents create fake identities to manipulate outcomes -- has not yet been studied. In this paper, we delve into the details of different cost-sharing mechanisms proposed in the literature, highlighting their non-Sybil-resistant nature. Furthermore, we prove no deterministic, anonymous, truthful, Sybil-proof, upper semicontinuous, and individually rational cost-sharing mechanism for public excludable goods is better than $\Omega(n)$-approximate. This finding reveals an exponential increase in the worst-case social cost in environments where agents are restricted from using Sybil strategies. To circumvent these negative results, we introduce the concept of \textit{Sybil Welfare Invariant} mechanisms, where a mechanism does not decrease its welfare under Sybil strategies when agents choose weak dominant strategies and have subjective prior beliefs over other players' actions. Finally, we prove that the Shapley value mechanism for symmetric and submodular cost functions holds this property, and so deduce that the worst-case social cost of this mechanism is the $n$th harmonic number $\mathcal H_n$ under equilibrium with Sybil strategies, matching the worst-case social cost bound for cost-sharing mechanisms. This finding suggests that any group of agents, each with private valuations, can fund public excludable goods both permissionless and anonymously, achieving efficiency comparable to that of non-anonymous domains, even when the total number of participants is unknown.ess and anonymously, achieving efficiency comparable to that of permissioned and non-anonymous domains, even when the total number of participants is unknown.

==> files/newproof.tex <==
\begin{lemma} Let $M$ be an anonymous, truthful, individually rational, upper semicontinuous, and Sybil-proof cost-sharing mechanism for constant cost functions. Then, for every agent $i$ and bid vector profile $\textbf{b}$ such that $x_i(\textbf{b})=1$ and $x_j(\textbf{b})=0$, then $x_i(\hat{\textbf{b}}_{j})=1$, where $\hat{\textbf{b}_j}=(b_1,...,b_{j-1},0,b_{j+1},...,b_n)$.
\end{lemma}
\begin{proof}
Assume that there exists a bid vector profile $\textbf{b} = (b_1, \ldots, b_n)$ such that $x_i(\textbf{b}) = 1$ and $x_j(\textbf{b}) = 0$, and also $x_i(\hat{\textbf{b}}_{j}) = 0$. Given that the mechanism is upper semicontinuous, there exists $\varepsilon > 0$ such that for $\textbf{b}' = (b_1, \ldots, b_i + \varepsilon, \ldots, b_n)$, the aforementioned properties hold. Now, assume that agents have valuations $\hat{\textbf{b}'}_j$. If agents report their true valuations, then agent $i$ receives a null allocation, resulting in zero utility. However, if agent $i$ reports an additional identity with bid $b_j$, then agent $i$ is allocated, with a payment $p \geq b_i$, leading to a utility of at least $\varepsilon > 0$. This situation implies that the mechanism is not Sybil-proof, which is a contradiction.
\end{proof}

Now, consider the following sequence:
\begin{equation*}
     v_n = \text{sup}_{v\geq 0}\{v\mid \textbf{x}(v_1-\varepsilon,...,v_{n-1}-\varepsilon,v) = \vec{0},\text{ for all }\varepsilon\in(0,\min\{v_{i}:i,...,n-1\})\}
\end{equation*}
Observe that since the mechanism is no-deficit, we have that $v_1\geq 1$. For a given $\varepsilon>0$, we define $\textbf{v}^n(\varepsilon):=(v_1-\varepsilon,...,v_n-\varepsilon)$.
\begin{proposition} For every $n$, $\max\{v_m:m\in[n]\}\leq 2v_n$.
\end{proposition}
\begin{proof} Let $m\in \text{argmax}\{v_m:m\in [n]\}$. If $v_m=v_n$, there is nothing to prove, so let's assume that $v_m>v_n$. Now, taking $v\in (v_n,v_m)$ there is an $\varepsilon>0$, such that the allocation $\textbf{b} = (v_1-\varepsilon,....,v_{n-1}-\varepsilon,v)$ is not null. By previous lemma, agents $n$ and $m$ are allocated, and so, if the agent $n$ reported $v_m$, it would also be allocated. Now suppose that agents from $i\in[n-1]\setminus\{m\}$, agents have valuation $v_i-\varepsilon$ and agent $m$ has valuation $v_m-\delta$, for $\delta\in(0,\min\{v_m-v_n,\varepsilon\})$. If the agent $m$ reports two identities with valuation $v_m-\varepsilon$, both are allocated and its payment per identity $p$ is at most $v$, since the mechanism is symmetric and the agent $n$ is allocated when the bid vector profile is $(v_1-\varepsilon,...,v_{n-1}-\varepsilon,v)$. Therefore, we have that the utility in this case is $v_m-\delta -2p\geq v_m-\delta-2v$. Since the mechanism is Sybil-Proof, the agent $m$ would rather report one bid with valuation $v_m-\delta$. However, the allocation of the bid vector profile $(v_1-\varepsilon,...,v_m-\delta,...,v_{n-1}-\varepsilon,0)$ is the null allocation, and so the utility of agent $m$ is zero. And so, $0\geq v_m-\delta-2v$. Making $\delta\rightarrow 0$ and $v\rightarrow v_n$, $2v_n\geq v_m$.
\end{proof}














\begin{lemma} \label{lemma:1} If a cost-sharing mechanism for constant cost functions is strong-monotonic, anonymous, truthful, individually rational, and Sybil-proof, then for every $\bb$, such that $b_i\geq b_j$, holds that $x_i(\bb)\geq x_j(\bb)$.
\end{lemma}
\textcolor{red}{Introduce $b_{-j}$}

\begin{proof} 



Let us prove it by contradiction. Suppose that there exists $\bb$ such that $b_i\geq b_j$, and $x_i(\bb)< x_j(\bb)$. The case where $b_i=b_j$ is not possible since the mechanism is symmetric and in particular holds the equal treatment property. Therefore, we will assume that $b_i>b_j$. Now, we have that $x_i(\bb)=0$ and $x_j(\bb)=1$. Since the mechanism is truthful, the map $x_j(\cdot,\textbf{b}_{-j})$ is monotone non-decreasing, and so, $x_j(b_i,\textbf{b}_{-j})=1$.


By strong monotonicity, $x_i(\bb_{-j},0)=0$. If the valuation vector profile is $\bb_{-j}$, then the utility of the player $i$ is zero. On the other hand, if the agent $i$ reports another Sybil with bid $b_j$, the public good is allocated to the agent since $j$ is his Sybil. By incentive compatibility, the $j$ identity pays at most $b_j$. So the total utility of the player reporting the bids $(b_i,b_j)$ is at least $b_i-b_j>0$, making the mechanism not Sybil-proof, leading to a contradiction.
\end{proof}
Now, consider the following sequence:
\begin{equation*}
     v_n = \text{sup}_{v\geq 0}\{v\mid \textbf{x}(v_1-\varepsilon,...,v_{n-1}-\varepsilon,v) = \vec{0},\text{ for all }\varepsilon\in(0,\min\{v_{i}:i,...,n-1\})\}
\end{equation*}
Observe that since the mechanism is no-deficit, we have that $v_1\geq 1$. For a given $\varepsilon>0$, we define $\textbf{v}^n(\varepsilon):=(v_1-\varepsilon,...,v_n-\varepsilon)$.

\begin{proposition}\normalfont Let $(\textbf{x},\textbf{p})$ be a individually rational, $\alpha(n)-$approximate, no-deficit, anonymous,  truthful, strong-monotonic, and Sybil-proof. Let $\{v_n\}_{n\in\mathbb N}$ be the sequence defined previously. Then:
\begin{enumerate}
    \item \label{item1} The sequence is well defined and is monotone non-increasing, i.e. $v_{n}\geq v_{n+1}$ for every $n\in\mathbb N$.
    \item \label{lemma:3} If $v_{n-1}>v_{n}$, then for every $v\in (v_n,v_{n-1})$, there exists $\delta>0$ such that for all $\varepsilon\in (0,\delta)$, the vector profile $(v_1-\varepsilon,...,v_{n-1}-\varepsilon,v)$ has allocation $S=[n]$.
    \item If $v_{n-1}>v_{n}$, then there exists a $\delta>0$ such that for every $\varepsilon\in (0,\delta)$ the bid vector profile $\textbf{w}^n(\varepsilon) = (v_1-\varepsilon,v_1-\varepsilon,...,v_{n}-\varepsilon)$ has the total allocation set, i.e. $S=[n]$.
    \item \label{lemma:4}For every $n$, it holds $v_1\leq 2v_n$.
    \item \label{lemma:5} It holds $\sum_{i=1}^n v_i\leq \alpha(n)$.
\end{enumerate}
\end{proposition}

\begin{proof} 1. If $\alpha(n)$ is finite, then it implies that the mechanism is consumer sovereign for $n$ players (otherwise the worst-case social cost would be infinite, see a similar proof in \cite{dobzinski2008shapley}). Therefore, $v_n$ must be finite for every $n$, otherwise, the worst-case social cost would be infinite, contradicting the fact that the mechanism holds the consumer sovereignty property. Now, let's prove that it is monotone non-increasing. First, for the bid vector profile $\textbf{w}=\textbf{v}^n(\varepsilon)$ no agent is assigned the public good by definition of $v_1,...,v_n$. Moreover, the bid vector profile with $l$ elements $(w_{i_1},...,w_{i_l})$, and $i_1,...,i_k\in [n]$ being pairwise different, also does not allocate the public good to any player. To prove it, consider the set $L=\{i_1,...,i_l\}$, then, the vector profile $\textbf{w} = (w_{i_1},...,w_{i_l},w_{-L})$ up to symmetry, and so has the same outcome since the mechanism is anonymous. Also, $\textbf{w}\geq (w_{i_1},...,w_{i_l},\vec{0}_{n-l})$, therefore since the mechanism is monotonic, we have that $x_{i_j}(w_{i_1},...,w_{i_l}) = x_{i_j}(w_{i_1},...,w_{i_l},\vec{0}_{n-l})=0$ for all $j=1,...,l$. Now lets use this to prove that $v_1\geq ...\geq v_n$. By contradiction, suppose not, let $i$ be the smallest element such that exist $j>i$ that $v_j>v_i$. 
Then, since the vector profile is $\textbf{v}^n(\varepsilon)$ no player has access to the public good, we have that $(v_1-\varepsilon,...,v_{i-1}-\varepsilon,v_j-\varepsilon)$ has also null allocation for all sufficiently small $\varepsilon>0$ by the previous argument. But this contradicts the fact that $v_i$ is the largest element that holds that the bid vector profile $(v_1-\varepsilon,...,v_{i-1}-\varepsilon,v)$ has the null allocation for all $\varepsilon>0$. Therefore, we have that the sequence is monotone decreasing. 

2. First, by definition, we have that the allocation of the bid vector profile $\textbf{v}^{n-1}(\varepsilon)$ is the empty set. Now, by definition of $v_n$, for every $v\in(v_n,v_{n-1})$, there exists $\delta>0$ such that for all $\varepsilon\in (0,\delta)$, the allocation of $(v_1-\varepsilon,...,v_{n-1}-\varepsilon,v)$ is not null. Since the sequence is non-increasing by Lemma \ref{lemma:1} we have that the allocation is a set $[k]$ for some $1\leq k\leq n$. Moreover, by strong-monotonicity, there is a $\delta>0$ such that for all $\varepsilon\in(0,\delta)$, the allocation set is $[k]$. Now, lets prove it by contradiction. Suppose that $S\not=[n]$. By the previous observations, we have that $k<n$, and we know that the allocation of the bid vector profile $(v_1-\varepsilon,...,v_k-\varepsilon)$ is null for all $\varepsilon>0$. If we assume that the valuation profile is $v_1-\delta/4,...,v_k-\delta/2$, we have that this reporting induces the null allocation, and so the first agent has $0$ utility. If the first player reports extra bids $v_{k+1}-\delta/2,...,v$, then the first player has access to the public good. On the other hand, the payment of the first identity is at most $v_1-\delta/2$ by Myerson lemma (since the first identity is the only Sybil identity that has access to the public good when the bid vector profile is $(v_1-\delta/2,...,v_{n-1}-\delta/2,v)$). Since the other identities are not served, their payment is $0$, and so the total utility of the player in this case is at least $v_1-\delta/4 -(v_1-\delta/2) = \delta/4>0$. Therefore, the mechanism would not be Sybil-proof, leading to a contradiction.

3. Observe that $\textbf{w}^n(\varepsilon)\geq (v_1-\varepsilon,...,v_n+\varepsilon)$ for sufficiently small $\varepsilon>0$. By the previous lemma, since the allocation of the second vector is $[n]$, we have, by strong monotonicity, that the allocation of the first vector is $[n]$.

4.  We will prove it by induction. The first case is trivial, since $v_1\leq 2v_1$. Now lets assume that it is true for $k<n$ and we will prove it for $n$. If $v_n=v_{n-1}$, then clearly $v_1\leq 2v_{n-1}=2v_n$, and so we can assume that $v_n<v_{n-1}$. 
By the 3 of proposition, there exists $\delta>0$ such that for every $\varepsilon\in (0,\delta)$ the bid vector profile $(v_1-\varepsilon,v_1-\varepsilon,....,v_{n-1}-\varepsilon)$ has full allocation. 
On the other hand, by definition of $v_{n-1}$ the bid vector profile $(v_1-\varepsilon,...,v_{n-1}-\varepsilon)$ is null for every $\varepsilon>0$, and so, the bid vector profile $(v_1-\varepsilon/2,v_2-\varepsilon,...,v_{n-1}-\varepsilon)$ also has the null allocation. Lets assume that the first player has valuation $v_1-\varepsilon/2$. If the first player reports two bids $v_1-\varepsilon$, we have that the bid vector profile is $(v_1-\varepsilon,v_1-\varepsilon,....,v_{n-1}-\varepsilon)$, having full allocation. By the point 2 of this proposition, we have that for every $v\in(v_n,v_{n-1})$ the bid vector profile $(v_1-\varepsilon,...,v_{n-1}-\varepsilon,v)$ has full allocation for sufficiently small $\varepsilon>0$. Therefore, by Myerson lemma, the payment $p_1$ of the Sybil identities of the player $1$ are, at most $v$. So, since the mechanism is Sybil-proof, we have that the utility of reporting without sybils is at least the one without Sybils and so $0\geq (v_1-\varepsilon/2)-2p_1\geq (v_1-\varepsilon/2)-2v$. When $v\rightarrow v_n$ and $\varepsilon\rightarrow0$, we get $2v_{n}\geq v_1$.

5. Since for all $\varepsilon>0$ it holds that $x(\textbf{v}^n(\varepsilon))=\vec{0}$, we have that the social cost is $\sum_{i=1}^n (v_i-\varepsilon)$. Since the mechanism is $\alpha(n)$-approximate, we have that $\sum_{i=1}^n (v_i-\varepsilon)\leq \alpha(n)$, making $\varepsilon\rightarrow0$, we have that $\sum_{i=1}^n v_i\leq \alpha(n)$.
\end{proof}

==> toimprove.tex <==



- IMPORTANT: 
\begin{itemize}
    \item How we can remove the symmetry of the cost function. How?
    \item How we can remove the strong-monotonicity assumption. Done!
    \item Explain Sybil extension simplier, may be move the categorial extension to the appendix.
    \item Statements are often imprecise, and assumptions are not clearly articulated.
    \item How can we anaylize randomized mechanisms?
\end{itemize}

https://aaai.org/aaai-conference/

